WorldPlanner: Monte Carlo Tree Search and MPC with Action-Conditioned Visual World Models

Robots must understand their environment from raw sensory inputs and reason about the consequences of their actions in it to solve complex tasks. Behavior Cloning (BC) leverages task-specific human demonstrations to learn this knowledge as end-to-end policies. However, these policies are difficult to transfer to new tasks, and generating training data is challenging because it requires careful demonstrations and frequent environment resets. In contrast to such policy-based view, in this paper we take a model-based approach where we collect a few hours of unstructured easy-to-collect play data to learn an action-conditioned visual world model, a diffusion-based action sampler, and optionally a reward model. The world model -- in combination with the action sampler and a reward model -- is then used to optimize long sequences of actions with a Monte Carlo Tree Search (MCTS) planner. The resulting plans are executed on the robot via a zeroth-order Model Predictive Controller (MPC). We show that the action sampler mitigates hallucinations of the world model during planning and validate our approach on 3 real-world robotic tasks with varying levels of planning and modeling complexity. Our experiments support the hypothesis that planning leads to a significant improvement over BC baselines on a standard manipulation test environment.

==> tables/consistency.tex <==
\begin{table}[t]
\label{tabel:consistency}
\begin{tabular}{@{}llll@{}}
\toprule
                          & $\sigma$                    & $2\sigma$      & $3\sigma$      \\ \midrule
\multicolumn{1}{|l|}{$x$} & \multicolumn{1}{l|}{$52\%$} & \multicolumn{1}{l|}{$52\%$} & \multicolumn{1}{l|}{$52\%$} \\ \midrule
\multicolumn{1}{|l|}{$y$} & \multicolumn{1}{l|}{$52\%$} & \multicolumn{1}{l|}{$52\%$} & \multicolumn{1}{l|}{$52\%$} \\ \midrule
$z$                       & $52\%$                      & $52\%$                      & $52\%$                      \\ \bottomrule
\end{tabular}
\end{table}
